Light-control of materials via nonlinear phononics

Nonlinear phononics is the phenomenon in which a coherent dynamics in a material along a set of phonons is launched after its infrared-active phonons are selectively excited using external light pulses. The microscopic mechanism underlying this phenomenon is the nonlinear coupling of the pumped infrared-active mode to other phonon modes present in a material. Nonlinear phonon couplings can cause finite time-averaged atomic displacements with or without broken crystal symmetries depending on the order, magnitude and sign of the nonlinearities. Such coherent lattice displacements along phonon coordinates can be used to control the physical properties of materials and even induce transient phases with lower symmetries. Light-control of materials via nonlinear phononics has become a practical reality due to the availability of intense mid-infrared lasers that can drive large-amplitude oscillations of the infrared-active phonons of materials. Mid-infrared pump induced insulator-metal transitions and spin and orbital order melting have been observed in pump-probe experiments. First principles based microscopic theory of nonlinear phononics has been developed, and it has been used to better understand how the lattice evolves after a mid-infrared pump excitation of infrared-active phonons. This theory has been used to predict light-induced switching of ferroelectric polarization as well as ferroelectricity in paraelectrics and ferromagnetism in antiferromagnets, which have been partially confirmed in recent experiments. This review summarizes the experimental and theoretical developments within this emerging field.

==> CR-gen.tex <==
%% 2019-03-25, second+epsilon alpha version 
%% CR style file, all series
%% Metadata
%  Journal title
\protected@edef\currentjournaltitle{Comptes Rendus. \CDRcrasseries}
%  journal publisher
\protected@edef\currentjournalpublisher{Acad\'emie des sciences, Paris}
%
%% The website
\def\CDRdomain{academie-sciences.fr/}
\xdef\journalURL{} % https://comptes-rendus.\CDRdomain\cdr@journaldirectory/}%
\def\CDRserviceName{centre Mersenne}
%
  \let\cdr@shortresps\@empty
  \let\cdr@resps\@empty
  \let\cdr@specialtitle@french\@empty
  \let\cdr@specialtitle@english\@empty
  \let\cdr@specialabstract@french\@empty
  \let\cdr@specialabstract@english\@empty
\let\cdr@presentedby\@empty
\def\PresentedBy#1{\gdef\cdr@presentedby{#1}}
\def\@set@presentedby{\cdr@presentedby@name\cdr@presentedby\@addpunct.}
\if@francais
\def\cdr@presentedby@name{Pr\'esent\'e par }
\else
\def\cdr@presentedby@name{Presented by }
\fi
%
\def\TopicFR#1{\gdef\cdr@topicFR{#1}}
\def\TopicEN#1{\gdef\cdr@topicEN{#1}}
\def\TopicEF#1#2{\gdef\cdr@topicEN{#1}\gdef\cdr@topicFR{#2}}
\def\RubricFR#1{\gdef\cdr@rubricFR{#1}}
\def\RubricEN#1{\gdef\cdr@rubricEN{#1}}
\def\RubricEF#1#2{\gdef\cdr@rubricEN{#1}\gdef\cdr@rubricFR{#2}}
%
%%geometry
\paperwidth=192truemm
\paperheight=262truemm
\ifx\undefined\pdfpagewidth\else
\pdfpagewidth\paperwidth
\pdfpageheight\paperheight
\fi
\setlength{\topmargin}{-12truemm}%
\setlength{\topskip}{13pt}
\setlength{\baselineskip}{12.2pt}
\setlength{\textheight}{\topskip}
\addtolength{\textheight}{48\baselineskip}%
%\textheight=210truemm
\headheight=10pt
\headsep 10mm
\marginparsep=10pt
\marginparpush=5pt
\marginparwidth=20mm
\footskip 14mm 

\pretolerance=600
\tolerance=2400 % INITEX sets this to 10000
\hbadness=2500
\vbadness=1000
\linepenalty=10
\hyphenpenalty=40
\exhyphenpenalty=50
\binoppenalty=700
\relpenalty=500
\clubpenalty=3000
\widowpenalty=4000 
\displaywidowpenalty=6000
\brokenpenalty=3000
\predisplaypenalty=10000
\doublehyphendemerits=600
\finalhyphendemerits=4000
\adjdemerits=10000
\emergencystretch=1.5em
\uchyph=1
\hfuzz.5pt
\lineskip=0pt 
%\calclayout
\long\def\MissingInfo#1{\textcolor{red}{#1}}

%% 
\normalparindent=12pt
\parindent=\normalparindent
\frenchspacing
%% ajust 10 pt interligne Fourier
\def\@mainsize{10}\def\@ptsize{0}%
  \def\@typesizes{%
    \or{5}{6}\or{6}{7}\or{7}{8}\or{8}{10.1}\or{9}{11.2}%
    \or{10}{12.2}% normalsize
    \or{\@xipt}{13}\or{\@xiipt}{14}\or{\@xivpt}{17}%
    \or{\@xviipt}{20}\or{\@xxpt}{24}}%
  \normalsize \linespacing=\baselineskip
%
%
\let\@listI\@listi
\@listi
%
%% Fonts
\ifcdr@m@nuscript
\IfFileExists{fourier.sty}{%
\PackageWarning{Mersenne/comptes Rendus}{Fourier font used}  
\usepackage{fourier}}
{\PackageWarning{Mersenne/comptes Rendus}{Fourier font not installed,
    the article will have to be retypeset!}}  
\else
\usepackage[expert]{fourier}
\pdfmapfile{=fourier.map}
\pdfmapfile{=fourier-utopia-expert.map}
\fi
\AtBeginDocument{\ifx\textsb\undefined\let\textsb\textbf\fi}
\def\@captionheadfont{\bfseries}%
\def\cdr@up{}%
%% Float captions
\captionindent=\normalparindent
\long\def\@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
    \captionseparator\@captionfont\cdr@up\enspace#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
%% unnumbered/unnamed captions
\def\silentcaption{%
   \ifx\@captype\@undefined
     \@latex@error{\noexpand\caption outside float}\@ehd
     \expandafter\@gobble
   \else
%     \refstepcounter\@captype
     \expandafter\@firstofone
   \fi
   {\@dblarg{\S@caption\@captype}}%
}
\long\def\S@caption#1[#2]#3{%
  \par
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
    {\protect\numberline{\ }{\ignorespaces #2}}%
  \begingroup
    \@parboxrestore
    \if@minipage
      \@setminipage
    \fi
    \normalsize
    \S@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
\long\def\S@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
%    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
%    \captionseparator\@captionfont\cdr@up\enspace
#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
% 
%% Page layout
\pagenumbering{arabic}%
%% 1st page
\def\ps@firstpage{\count@=\currentyear
  \ps@plain
  \def\@oddfoot{{\scriptsize    
     % ISSN (electronic) : \@Eissn\hfill\texttt{\url{\journalURL}}
}}
  \let\@evenfoot\@oddfoot
  \def\@oddhead{\@serieslogo\hss}%
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
%% Identificiation article 1st page
\def\prepageinfo{p.\, }
\def\pageinfosep{-} 
\def\printDOI{\ifx\CDRdoi\@empty
  \MissingInfo{DOI unassigned
    yet}\else\url{https://doi.org/\CDRdoi}\fi}
\def\@logofont{\footnotesize} 
\def\article@logo{%
  \set@logo{\hsize\textwidth%
    {\Large\textit{Comptes Rendus\\
        \CDRcrasseries}\\[2pt]} 
    \ifcdr@m@nuscript%
    % When authors submit a manuscript with option manuscript, don't
    % bother with publication data 
     \textbf{Draft}
    \else 
      \ifnum\currentvolume>\z@\textbf{\currentyear}, 
       % This tests whether this is a regular issue, or "To appear" preview,
       % where the value is 0. The following is the regular case
       \currentvolume, \no \currentissue, \prepageinfo\pageinfo
      \else 
       % This is for "To appear" case
       Article to appear%
       \ifx\@empty\@dateposted\else, 
        % If a dateposted is provided, use it. Maybe we should print a warning
        % in any case.
        posted online
        {\selectlanguage{english}\printdate{\@dateposted}}
       \fi
      \fi	
    \\\texttt{\printDOI}
    \fi
    \hfill\raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}\\[18bp]
    \centerline{\rule{.8\textwidth}{1.5bp}}
%    \vspace*{10pt}
}}% end \article@logo
%
%%  Copyright
\def\@setcopyright{}%
%% Standard pages
\def\ps@headings{\ps@empty
  \def\@evenhead{%
    \setTrue{runhead}%
    \rlap{\thepage}{}%\scshape
    \footnotesize\def\lastname####1{%\textsc
      {####1}}%
    \hfil
    \def\thanks{\protect\thanks@warning}%
    \TopAuthors{}{}\hfil}%
  \def\@oddhead{%
    \setTrue{runhead}%
    \let\\\relax
    \hfil
    \def\thanks{\protect\thanks@warning}%
    % {\footnotesize\itshape\rightmark{}{}}\hfil
    % \llap{\thepage}{}%
    {\footnotesize\TopAuthors{}{}}\hfil
    \llap{\thepage}{}%
  }%
  \let\@mkboth\cdr@markboth
  \def\@oddfoot{%
%    \scriptsize\textit{\shortpublname}\ifcdr@m@nuscript---Draft, \today\else,
%      \ifnum\currentvolume=\z@\the\year\else\textbf{\currentyear}, \currentvolume,
%        \no\currentissue, \pageinfo\fi\fi\hfil
    }%
  \let\@evenfoot\@oddfoot
}
%
\def\currentyear{0000}

%% Alternative code for title/editors of special volumes
%% To be evaluated later
% \ifcdr@volume
%  \def\maketitle{%\@makePDFinfo
%   \def\cdrsom@out@filename{\cdr@idvol.cdrsom}%
%   \@makeSOM
%  } 
%  \def\enddoc@text{}
% \else
%   \let\cdr@specialvolshortresps\@empty
%   \let\cdr@specialvolresps\@empty
%   \let\cdr@specialvoltitle@french\@empty
%   \let\cdr@specialvoltitle@english\@empty
%   \let\cdr@specialvolabstract@french\@empty
%   \let\cdr@specialvolabstract@english\@empty
% \AtBeginDocument{%
% \begingroup\makeatletter
% \newcommand\SomLine[9]{%
%   \gdef\cdr@specialvolshortresps{#1}%
%   \gdef\cdr@specialvolresps{#2}%
%   \gdef\cdr@specialvoltitle@french{#5}%
%   \gdef\cdr@specialvoltitle@english{#4}%
%   \gdef\cdr@specialvolabstract@french{#7}%
%   \gdef\cdr@specialvolabstract@english{#6}%
%   }%
% \InputIfFileExists{../\CDRidvol.cdrsom}{%
% \message{** Fichier  \CDRidvol.cdrsom charg\'e pour
%   cet article **^^J}}{%
% \message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
% \makeatother\endgroup}
% \fi

\pagestyle{headings}%
%
\setlength{\@titletopskip}{26\p@}
\setlength{\@titlebotskip}{0\p@}
%% title presentation 
\def\CDRtitleSep{\,/\,}%
\def\@settitle{%
  \begin{flushleft}
 \vspace*{10pt}

 \strut
\ifx\TITREspecial\@empty\else 
% This is part of a thematic issue
  \Large
    \ifx\cdr@specialtitle@english\@empty
       \MissingInfo{Thematic issue title missing!}
    \else
        %% only english special title
       \cdr@specialtitle@english%
       \ifx\cdr@specialtitle@french\@empty\else
        %% add French special title
        \CDRtitleSep{\itshape\cdr@specialtitle@french}
       \fi
    \fi
\fi      
    \vspace*{4pt}
 
%    \strut
    \@setTopicORRubric

   \addvspace{10pt}

   \def\baselinestretch{1.2}\large%\vfil
   {\Huge%\itshape
     \@title\par}

    {\huge\itshape

      \ifx\@alttitle\@empty\else   

      \vspace*{14pt}

      \@alttitle\par\fi}
 
    \vspace*{16pt}

  \end{flushleft}%
}
%
\def\CDRtopicSep{\,/\,}%
\def\CDRrubricSep{\,/\,}%
\def\@setTopicORRubric{%
\if@francais
   \ifx\cdr@topicFR\@empty
% rubric and topic mutually exclusive
     \ifx\cdr@rubricFR\@empty\else
       {%\textbf
       {%\itshape
         \large\cdr@rubricFR\ifx\cdr@rubricEN\@empty\else\CDRrubricSep%
         \itshape\cdr@rubricEN\fi}}%
     \fi
   \else
    {%\textbf
      {%\itshape
        \large\cdr@topicFR\ifx\cdr@topicEN\@empty\else\CDRtopicSep%
         \itshape\cdr@topicEN\fi}}%
   \fi
  \else
   \ifx\cdr@topicEN\@empty
% rubric and topic mutually exclusive
     \ifx\cdr@rubricEN\@empty\else
       {%\textbf
       {%\itshape
         \large\cdr@rubricEN\ifx\cdr@rubricFR\@empty\else\CDRrubricSep%
         \itshape\cdr@rubricFR\fi}}%
     \fi
   \else
    {%\textbf
      {%\itshape
        \large\cdr@topicEN\ifx\cdr@topicFR\@empty\else\CDRtopicSep%
         \itshape\cdr@topicFR\fi}}%
   \fi
  \fi
}

\let\@ESM\@empty
\newcommand\ESM[1]{\def\@ESM{#1}}

\def\cdr@preabstracthook{\par
  \bigskip}%
%   {\abstractfont\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@%
%   \ifx\@empty\@dateaccepted \MissingInfo{This article is a draft (not yet accepted!)}%
%   \else \@setdate\fi}\par\bigskip
% }}
\def\cdr@interabstracthook{\par}%\smallskip}
\def\cdr@postabstracthook{\par
  \ifx\@empty\@keywords\else\@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setkeywords}\smallskip\fi
  \ifx\@empty\@altkeywords\else \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setaltkeywords}\smallskip\fi
  \ifx\@empty\@subjclass\else \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setsubjclass}\smallskip\fi
  \ifx\@empty\thankses\else
  \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setthanks}\smallskip\fi%
  \ifx\@empty\@ESM\else
  \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setESM}\smallskip\fi%
  \par\medskip
  {\abstractfont\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@%
   \@setdate}\par\bigskip}%
 \vskip24pt plus 8pt}
%
\def\CDRextrafirstfootnotetext{}
\def\abstractheadfont{\bfseries}
\def\@setabstracthead{{\abstractheadfont\abstractname\unskip.\kern.25em\ignorespaces}}
\def\@setaltabstracthead{{\abstractheadfont\altabstractname\unskip.\kern.25em\ignorespaces}%
}
%
%% authors
\def\@firstauthor#1\and#2\stop{#1}
\def\shortrunauthors{\gdef\@maketitle@shortauthors@hook{\def\topauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
\def\shortrunPDGauthors{\g@addto@macro\@maketitle@shortauthors@hook{\def\PDGauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
 \if@francais
  \def\manuscriptname{Manuscrit}%
  \def\receivedname{re\c cu}%
  \def\revisedname{r\'evis\'e}%
  \def\acceptedname{accept\'e}%
  \def\@@and{et}%
 \else
  \def\manuscriptname{Manuscript}%
  \def\receivedname{received}%
  \def\revisedname{revised}%
  \def\acceptedname{accepted}%
  \def\@@and{and}%
 \fi
%
\AtBeginDocument{\ifx\@daterevised\@dateaccepted\global\cdr@revisedacceptedtrue\fi
\ifx\@datereceived\@dateaccepted\global\cdr@receivedacceptedtrue\fi}
%
%%%%% presentation auteurs 
%\def\@@and{\&}
 \def\author@andify{%
   \nxandlist {\unskip ,\penalty-2 \space\cdr@count@hasaddr=\z@\ignorespaces}%
     {\unskip {} \cdr@count@hasaddr=\z@\@@and~}%
     {\unskip {} \penalty-2  \cdr@count@hasaddr=\z@\@@and~}%
 }
% \def\@maketitle@shortauthors@hook{\msia@shortauthor@andify\shortauthors\let\topauthors\shortauthors}
\newcount\cdr@thankcount
\cdr@thankcount\z@
\ifcdr@ltxgrid\else
\def\@alph#1{\ifcase#1\or a\or b\or c\or d\else\@ialph{#1}\fi}
\def\@ialph#1{\ifcase#1\or \or \or \or \or e\or f\or g\or h\or i\or j\or
 k\or l\or m\or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or x\or
 y\or z\or aa\or bb\or cc\or dd\or ee\or ff\or gg\or hh\or ii\or jj\or
 kk\or ll\or mm\or nn\or oo\or pp\or qq\or rr\or ss\or tt\or uu\or
 vv\or ww\or xx\or yy\or zz\else\@ctrerr\fi}
\fi
\def\cdr@CorrespondingAuthorIs{0}
\def\CDRorcid#1{\relax}
\let\IsEqualContrib\relax
\newcount\ContrA\ContrA=\z@
\let\IsCorresp\relax
\newcount\CorrA\CorrA=\z@
\def\display@orcid#1{%
  \href{https://orcid.org/#1}{%
    \raisebox{.7ex}[0pt][0pt]{%
%      \includegraphics[height=1.1ex]{orcid.png}{}%
      \includegraphics[height=1.1ex]{orcid-bw.png}}%
%{\usefont{TU}{academicons}{m}{n}\symbol{"E9D9}}}%
    }
}
\newcount\cdr@count@hasaddr\cdr@count@hasaddr=\z@%
\def\@setauthors{%
  \begingroup
  \def\CDRorcid##1{\kern1pt\display@orcid{##1}}%
  \def\IsCorresp{\textsuperscript{$*$,}\global\advance\CorrA\@ne\relax}%
  \def\IsEqualContrib{\textsuperscript{$\#$,}\global\advance\ContrA\@ne\relax}%}%
  \def\thanks{\protect\thanks@warning}%
  \author@andify\authors
  \def\\{\space}%
  \def\Same{\same}%
  \def\New{\new}%
  \def\hasaddress##1##2{%
    \ifnum\cdr@count@hasaddr=\z@\kern.1em\fi
    \@ifempty{##1}{% cas pas sameaddress
%% increment de compteur
\global\advance\cdr@thankcount\@ne%
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\cdr@thankcount}}%
}{% cas sameaddress
\def\What{##1}\ifx\What\Same
%% pas d'increment de compteur
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\cdr@thankcount}}%
\else\ifx\What\New
%% increment de compteur
\global\advance\cdr@thankcount\@ne%
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\cdr@thankcount}}%
\else
%% manual numbering mode, produced by addressSameAs
\count@=##1\relax
\textsuperscript{\ifnum\cdr@count@hasaddr>\z@, \fi
  \textit{\@alph\count@}}%
\fi\fi}\advance\cdr@count@hasaddr\@ne}%
%\begin{minipage}[t]{.9\linewidth}\raggedright
\begingroup\hsize=.9\linewidth\raggedright
\large\textsb{\authors}\hfill\break%
  \ifx\@empty\contribs \else \\\penalty-3 \space \@setcontribs
  \@closetoccontribs \fi
  \par
  \endgroup
%\end{minipage}
\endgroup
  \ifnum\CorrA=\z@\else{{\def\@thefnmark{\rule{0pt}{10pt}$*\,$}%
    \@footnotetext{\def\CDRss{\ifnum\CorrA>\@ne\relax s\fi}\if@francais
      Auteur\CDRss\ correspondant\CDRss\else Corresponding
      author\CDRss\fi. \CDRextrafirstfootnotetext}}}\fi
  \ifnum\ContrA=\z@\else{{\def\@thefnmark{\rule{0pt}{10pt}$\#\,$}%
    \@footnotetext{\if@francais
      Contributions \'egales\else Contributed equally\fi.}}}\fi
}%
\def\@setafterauthor{%
  \vglue3mm%
%  \hspace*{0pt}%
\begingroup\hsize=10cm\raggedright
\noindent
%\hspace*{\abstractmarginL}\begin{minipage}[t]{10cm}
   \leftskip\abstractmarginL
  \normalfont\Small
  \@afterauthor\par
\endgroup
\vskip2pt plus 3pt minus 1pt
}
\def\@afterauthor{\ifx\@empty\addresses \else\@setaddresses\par
\ifcdr@emails\ifcdr@existcurraddr\@setcurraddr\par\fi
\@setemails\par\fi
  \bigskip%
  \fi}
\newif\ifcdr@existcurraddr\cdr@existcurraddrfalse
\def\@setaddresses{%\par
  \begingroup
  \cdr@thankcount\z@
   \ifcdr@hyperref  \url@samestyle
   \else\def\url##1{##1}%
   \def\href##1##2{##2}\fi
   \def\affiliationonly##1{##1}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{##1\@addpunct.\@par}
   \def\hasaddress##1{\relax}%
   \def\author##1{%\ifnum\cdr@notes@adress=\z@\else\@@par\indent\fi\global\advance\cdr@notes@adress1
     % \textsuperscript{\@alph\cdr@notes@adress}\kern.2em
     \def\\{ \ignorespaces}\ignorespaces}%
   \def\address##1##2{\begingroup
   \@ifempty{##1}{% cas pas addressSameAs
     \ifnum\cdr@thankcount>\z@\par\vskip4pt\fi\global\advance\cdr@thankcount\@ne
     \textsuperscript{\textit{\@alph\cdr@thankcount}}\kern.2em{\ignorespaces##2\unskip}}{}\endgroup}%
   \def\curraddr##1##2{%% Showing emails authorwise? Let's assume this follows the same logic as emails grouping.
     \ifcdr@emails\global\cdr@existcurraddrtrue\else
     \begingroup
     \@ifnotempty{##2}{\@@par\curraddrname{}\textit{\thsp:} %
       {\ignorespaces##2\unskip}\endgroup}\fi}%
   \def\email##1##2{%% Showing emails authorwise?
     \ifcdr@emails\else
     \begingroup
     \@ifnotempty{##2}{\@@par\emailaddrname{}%
       \@ifnotempty{##1}{ (##1)}\textit{\thsp:} %
       \href{mailto:##2}{##2}}\endgroup\fi
   }%
   \def\urladdr##1##2{\begingroup
%     \def~{\char`\~}%
     \@ifnotempty{##2}{\@@par\urladdrname{}\textit{\thsp:} %
       \url{##2}}\endgroup}%
   \addresses%\@addpunct.%
   \endgroup
 }
\def\@setemails{%\par
  \begingroup
   \cdr@thankcount\z@
   \ifcdr@hyperref  \url@samestyle
   \else\def\url##1{##1}%
   \def\href##1##2{##2}\fi
   \def\affiliationonly##1{\relax}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{\relax}
   \def\hasaddress##1{\relax}%
   \def\author##1{}%\ifnum\cdr@thankcount=\z@\else, \fi}
   \def\address##1##2{\relax}%
   \def\curraddr##1##2{\relax}%
   \def\email##1##2{%% Showing emails authorwise?
     \ifcdr@emails
     \begingroup
     \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi\href{mailto:##2}{##2}\@ifnotempty{##1}{ \mbox{(##1)}}}\endgroup\fi
     \global\advance\cdr@thankcount\@ne}%
   \def\urladdr##1##2{\relax}%
   \sbox\@tempboxa{\addresses\xdef\CDRess{\ifnum\cdr@thankcount>\@ne\relax s\fi}}%
   \ifdim\wd\@tempboxa>1em\relax
   \vskip2pt\@@par\textit{\emailsaddrname{}\CDRess\thsp:} 
   \cdr@thankcount\z@
   \addresses%\@addpunct.%
   \fi
   \endgroup
 }
\def\@setcurraddr{%\par
  \begingroup
   \cdr@thankcount\z@
   \ifcdr@hyperref  \url@samestyle
   \else\def\url##1{##1}%
   \def\href##1##2{##2}\fi
   \def\affiliationonly##1{\relax}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{\relax}
   \def\hasaddress##1{\relax}%
   \def\author##1{}%\ifnum\cdr@thankcount=\z@\else, \fi}
   \def\address##1##2{\relax}%
   \def\curraddr##1##2{%% Showing current addresses?
     \ifcdr@emails
     \begingroup
     \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi##2\@ifnotempty{##1}{ \mbox{(##1)}}}\endgroup\fi
     \global\advance\cdr@thankcount\@ne}%
   \def\email##1##2{\relax}%
   \def\urladdr##1##2{\relax}%
   \sbox\@tempboxa{\addresses\xdef\CDREss{\ifnum\cdr@thankcount>\@ne\relax es\fi}}%
   \ifdim\wd\@tempboxa>1em\relax
   \vskip2pt\@@par\textit{\curraddrname{}\CDREss\thsp:} 
   \cdr@thankcount\z@
   \addresses%\@addpunct.%
   \fi
   \endgroup
 }
%%%% Fin pres aut

%% Footnotes 1st page
\def\@adminfootnotes{}%
%   \let\@makefnmark\relax  \let\@thefnmark\relax
%   \begingroup\normalparindent0pt\footnotesep10pt\relax
%\endgroup}
\def\@setsubjclass{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\subjclassname.}\kern.25em\ignorespaces
  \@subjclass\@addpunct{{\upshape.}}\par}
\RequirePackage[english,iso]{isodate}
\origdate
\RequirePackage[shortlabels]{enumitem}  
\setlist{font=\upshape}
\newif\ifcdr@revisedaccepted\cdr@revisedacceptedfalse
\newif\ifcdr@receivedaccepted\cdr@receivedacceptedfalse
\def\datererevised#1{\def\@datererevised{#1}}%
\let\@datererevised\@empty
\def\daterevisedaccepted#1{\def\@daterevised{#1}\def\@dateaccepted{#1}\cdr@revisedacceptedtrue}
%
 \def\@setdate{%
   \ifx\@empty\@dateaccepted \MissingInfo{} %This article is a draft (not yet accepted!)}%
   \else 
  \if@francais
    \itshape\selectlanguage{french}%
    \noindent Manuscrit \ifx\@empty\cdr@presentedby\else pr\'esent\'e
    par \cdr@presentedby, \fi re\c cu  
      \ifcdr@receivedaccepted et accept\'e le \printdate\@datereceived
      \else
        le \printdate\@datereceived,
        \ifcdr@revisedaccepted	
           r\'evis\'e et  accept\'e le \printdate\@dateaccepted
        \else
          \ifx\@empty\@daterevised
          \else
            r\'evis\'e le \printdate\@daterevised
              \ifx\@empty\@datererevised
              \else\ et le \printdate\@datererevised
              \fi, 
          \fi
          accept\'e le \printdate\@dateaccepted
        \fi
      \fi.
  \else
    \itshape\selectlanguage{english}%
    \noindent Manuscript \ifx\@empty\cdr@presentedby\else presented
    by \cdr@presentedby, \fi received
    \ifcdr@receivedaccepted and accepted \printdate\@datereceived
    \else
     \printdate\@datereceived,
     \ifcdr@revisedaccepted
      revised and  accepted  \printdate\@dateaccepted
     \else
      \ifx\@empty\@daterevised
      \else
        revised  \printdate\@daterevised
        \ifx\@empty\@datererevised
        \else\ and
         \printdate\@datererevised
        \fi,
      \fi
       accepted  \printdate\@dateaccepted
     \fi
     \fi.
   \fi
\fi}
\ifcdr@thematicissue
\AtBeginDocument{%
\let\@datereceived\@empty
\let\@daterevised\@empty
\let\@dateaccepted\@empty
\let\@datererevised\@empty
}
\def\@setdate{}
\fi
%
\def\dedicatoryfont{\normalfont\footnotesize\itshape}
\def\@setdedicatory{%
    \begingroup
      \def\signature##1{\nobreak\hskip 2em plus 1fil
        \penalty-5\hbox{}\nobreak\hfil\parfillskip=0pt
        \mbox{\upshape ##1}\par}
      \raggedleft
      \dedicatoryfont
      \@dedicatory\par
    \endgroup}
\def\@setkeywords{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\keywordsname.}\kern.25em\ignorespaces
  \@keywords\@addpunct{{\upshape.}}\par}
\def\@setaltkeywords{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\altkeywordsname.}\kern.25em\ignorespaces
  \@altkeywords\@addpunct{{\upshape.}}\par}
\newcount\cdr@numberofthanks\cdr@numberofthanks=\z@
\def\@setthanks{\abstractfont\def\thanks##1{\ifnum\cdr@numberofthanks=\z@\relax\else\@par
   \fi##1\@addpunct{{\upshape.}}\advance\cdr@numberofthanks1\relax}{\abstractheadfont\thanksname.}\kern.25em\ignorespaces\thankses\par}
\def\@setESM{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\ESMname.}\kern.25em\ignorespaces
  \@ESM\@addpunct{{\upshape.}}\par}
\def\@settranslators{\par
  \begingroup
  \translatedby\ \andify\@translators
  {\sl \ignorespaces\@translators} \@@par
  \endgroup}
\if@francais
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Mots-cl{\'e}s}
\def\altkeywordsname{Keywords}
\def\subjclassname{Classification math{\'e}matique par sujets (2010)}
\def\thanksname{Financement}
\def\emailsaddrname{Courriel}
\def\ESMname{Mat{\'e}riel {\'e}lectronique suppl{\'e}mentaire}
\else
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Keywords}
\def\altkeywordsname{Mots-cl{\'e}s}
\def\subjclassname{Mathematical subject classification (2010)}
\def\thanksname{Funding}
\def\emailsaddrname{E-mail}
\def\ESMname{Electronic supplementary material}
\fi
\@xp\let\csname subjclassname@2010\endcsname \subjclassname
%
\def\longthankssection{\subsubsection*{Acknowledgements}}
\long\def\longthanks#1{\longthankssection

  #1}%
%
%
\def\enddoc@text{}
%
%% Page de garde
\def\@makePagedeGarde{%
\ifcdr@pagedegarde
{\makeatletter\input{CR-pagedegarde}}%
\newpage\ifcdr@HTML\pagecolor{white}\else\gdef\GPT@pageliteral{}\fi\fi}
%
\ifcdr@sommaire
\let\cdr@postabstracthook\@empty
\def\ps@firstpage{\count@=\currentyear
  \ps@plain
  \let\@oddfoot\@empty
  \let\@evenfoot\@oddfoot
  \def\@oddhead{\@serieslogo\hss}%
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
\let\ps@headings\ps@empty
\let\ps@plain\ps@empty
\def\article@logo{%
  \set@logo{\hsize\textwidth%
 {\Large\textit{Comptes Rendus\\
        \CDRcrasseries}\\[2pt]} \ifx\@empty\currentvolume
    \textbf{Draft}
    \else \textbf{\currentyear},
    \currentvolume\ifx\currentissue\@empty\else, \no
    \currentissue\fi\fi\\
\mbox{}   \hfill\raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}\\[18bp]
    \centerline{\rule{.8\textwidth}{1.5bp}}
  }%
}
%
\def\smfbyname{\vspace*{-17mm}}
\def\lastname#1{#1}
\def\junior#1{\unskip, #1}%
\renewcommand{\@pnumwidth}{4.5em}
\def\@adminfootnotes{}
\def\enddoc@text{}
%% 
\fi
\ifcdr@volume
%\RequirePackage{url}
\def\@makefront{%
  \IncludeSom{\cdr@journalacro -Sommaire}%
  \cleardoublepage
  \ifcdr@SOM
    \@makeSOM
\begingroup\makeatletter
\newcommand\SomLine[9]{%
  \gdef\cdr@shortresps{##1}%
  \gdef\cdr@resps{##2}%
  \gdef\cdr@specialtitle@french{##5}%
  \gdef\cdr@specialtitle@english{##4}%
  \gdef\cdr@specialabstract@french{##7}%
  \gdef\cdr@specialabstract@english{##6}%
  }%
\InputIfFileExists{./\CDRidvol.cdrsom}{%
\message{** Fichier  \CDRidvol.cdrsom charge  **^^J}}{%
\message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
\makeatother\endgroup
\fi
}
\def\@makebody{%
  \ifcdr@newsom
  \immediate\write18{rm -f \cdr@journalacro -Sommaire-data.tex}%
  \fi
% \ifcdr@specialtitre
%   \newwrite\cdr@globalcfgfile
%   \immediate\openout\cdr@globalcfgfile=\CDRidvol -global.cfg
%   \immediate\write\cdr@globalcfgfile{\the\cdr@specialtitret}%
%   \immediate\closeout\cdr@globalcfgfile
% \fi
  \pagenumbering{arabic}%
  \setcounter{page}{\@FirstPage}%
  \tkkp={\setpage}%
}

\def\enddoc@text{}

\else\ifcdr@sommaire %% Sommaire
\AtEndOfClass{%
 \begingroup\makeatletter
 \newcommand\SomLine[9]{%
  \gdef\cdr@shortresps{#1}%
  \gdef\cdr@resps{#2}%
  \gdef\cdr@specialtitle@french{#5}%
  \gdef\cdr@specialtitle@english{#4}%
  \gdef\cdr@specialabstract@french{#7}%
  \gdef\cdr@specialabstract@english{#6}%
  }
 \InputIfFileExists{./\CDRidvol.cdrsom}{%
  \message{** Fichier  \CDRidvol.cdrsom charge  **^^J}%
%  \let\SomLine\undefined
  }%
  {%
  \message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
 \makeatother\endgroup}
\AtBeginDocument{%
 \newcommand\SomLine[9]{%
\def\lng{#3}\def\LNG{french}%
  \par \addpenalty\@secpenalty\addvspace{\medskipamount}%
    \begingroup\hyphenpenalty50\def\\{\allowbreak}%
	\parindent0pt
%    \parindent-\normalparindent \leftskip\normalparindent\relax 
    \rightskip\@pnumwidth% plus6em
    {\bfseries\ignorespaces#2\unskip}\@par
	 \parfillskip-\@pnumwidth
%    \hskip1em
\ifx\lng\LNG#5\else#4\fi\unskip\leavevmode
                              %
    \nobreak\hskip2pt\nobreak \leaders\hbox{$\m@th \mkern 1.5mu\hbox{.}\mkern
      1.5mu$}\hfill \nobreak
     \hb@xt@\@pnumwidth{\@tocpagenum{\ignorespaces#8\unskip-\ignorespaces#9\unskip}}%
     \par
    \endgroup
%    \begingroup\parindent\normalparindent\relax\leftskip2.4em\footnotesize\ignorespaces#7\unskip\par
%    \endgroup
}
}
\else %% Articles
\AtEndOfClass{%
\begingroup\makeatletter
\newcommand\SomLine[9]{%
  \gdef\cdr@shortresps{#1}%
  \gdef\cdr@resps{#2}%
  \gdef\cdr@specialtitle@french{#5}%
  \gdef\cdr@specialtitle@english{#4}%
  \gdef\cdr@specialabstract@french{#7}%
  \gdef\cdr@specialabstract@english{#6}%
  }%
\InputIfFileExists{../\CDRidvol.cdrsom}{%
\message{** Fichier  \CDRidvol.cdrsom charge pour
  cet article **^^J}}{%
\message{** Pas de fichier \CDRidvol.cdrsom  pour ce volume !**^^J}}%
\makeatother\endgroup}

\fi\fi

%AJOUTS CS
%\RequirePackage{amssymb,upref}

\NumberTheoremsIn{}
\setcounter{tocdepth}{3}

%% Thms
\ifcdr@cdrthmdefs\OneNumberAllTheorems\fi
\def\th@plain{%
  \thm@bodyfont{\normalfont\itshape}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em\ignorespaces}%
  \let\thm@indent\noindent 
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
  \itshape
}
\def\th@remark{%
  \thm@bodyfont{\normalfont}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em}%
  \let\thm@indent\noindent 
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
}
\let\th@definition\th@plain
%\def\cdr@proofindent{\z@}%{1.5\parindent}
\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\cdr@proofindent
        {\providecommand\printref{\relax}%
\bfseries
    #1\@addpunct{\cdr@proofpunct}}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
%% Sectionning 
\def\@startsection#1#2#3#4#5#6{%
 \if@noskipsec \leavevmode \fi
 \par \@tempskipa #4\relax
 \@afterindenttrue
 \ifdim \@tempskipa <\z@ \@tempskipa -\@tempskipa \@afterindentfalse\fi
 \if@nobreak \everypar{}\else
     \addpenalty\@secpenalty\addvspace\@tempskipa\fi
 \@ifstar{\@dblarg{\@sect{#1}{\@m}{#3}{#4}{#5}{#6}}}%
         {\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}%
}
\def\@seccntformat#1{%
  \protect\textup{\protect\@secnumfont
    \csname the#1\endcsname
    \protect\@secnumpunct
  }%
}
\def\@sectionfamily{\normalfont}
\def\@sectionfont{\@sectionfamily\large\bfseries}
\let\contentsnamefont\@sectionfont
\def\@secnumfont{\selectfont}
%\def\@upn{\normalfont\selectfont}
\def\@subsectionfont{\@sectionfamily\large\itshape}
\def\@subsubsectionfont{\@sectionfamily\itshape}
\def\@paragraphfont{\normalfont\bfseries}


\def\section{\@startsection{section}{1}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\@sectionfont}}
\def\subsection{\@startsection{subsection}{2}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\normalfont\@subsectionfont}}
\def\subsubsection{\@startsection{subsubsection}{3}%
  \z@{.5\linespacing\@plus.5\linespacing}{.5\linespacing}%
  {\normalfont\@subsubsectionfont}}
\def\paragraph{\@startsection{paragraph}{4}%
  \z@{.5\linespacing\@plus.5\linespacing}{-\fontdimen2\font}%
  {\normalfont\@paragraphfont}}
%
\newcount\tochyphenpenalty
\tochyphenpenalty\@M
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\tochyphenpenalty
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax
      \advance\leftskip\@tempdima\relax
    \advance\rightskip\@pnumwidth % plus1em
    \parfillskip-\@pnumwidth
    {#5{\leavevmode\hskip-\@tempdima #6}}%
    \nobreak
    \xleaders\hbox to1ex{\normalfont\hss.\hss}\hfil\nobreak
    \hbox to\@pnumwidth{\@tocpagenum{#7}}\par
    \nobreak
    \endgroup
  \fi}
%
\renewcommand{\tocpart}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 #2.\kern1ex}}#3}
\let\tocsection\tocpart
\let\tocsubsection\tocsection
\let\tocsubsubsection\tocsection
\let\tocparagraph\tocsection
\def\l@part{\@tocline{-1}{12pt plus2pt}{0pt}{}{\bfseries\smf@boldmath}}
\def\l@section{\@tocline{1}{0pt}{0pc}{}{}}
\def\l@subsection{\@tocline{2}{0pt}{1pc}{}{}}
\def\l@subsubsection{\@tocline{3}{0pt}{2pc}{}{}}
\def\l@paragraph{\@tocline{5}{0pt}{3pc}{}{}}
\def\l@figure{\@tocline{0}{3pt plus2pt}{0pt}{}{}}
\let\l@table\l@figure
%
\def\@smfprotect{\let\smfcr\\\def\\{\protect\smfcr}}
\DeclareRobustCommand{\MakeUppercase}[1]{{%
    \@smfprotect\upchars@
    \protected@edef\reserved@a{#1}\uppercasenonmath\reserved@a\reserved@a}}
\protected@edef\MakeUppercase#1{\MakeUppercase{#1}}
%
% \def\@makefnmark{%
%   \leavevmode
%   \raise.9ex\hbox{\fontsize\sf@size\z@\normalfont(\@thefnmark)}%
% }%CS
%
%% Additional macros %%
\AtBeginDocument{%
\csname url@samestyle\endcsname
\begingroup
\ifx\@dateposted\@empty
 % no known date posted at begin doc
 \ifnum\currentvolume=\z@%
  % if we are creating a vol. 0, then we generate and save the current
  % date as dateposted
  \def\setpdftimes#1#2{\gdef\@dateposted{#2}}%
  \InputIfFileExists{\jobname -pdftimestamp.txt}{}{}%
  \toks@{\dateposted}
  \immediatelywrite@shell{echo \cdr@lq\the\toks@{\@dateposted}\cdr@rq 
    >  \jobname -dateposted.txt}%
 \else
  % if we are preparing a regular volume, then we get a previously
  % stored date, if any
   \InputIfFileExists{\jobname -dateposted.txt}{}{}%
 \fi
\fi
\endgroup
}
\emergencystretch2em
\arraycolsep 1.5pt
%%
\def\etal{{\normalfont\itshape et al.}}

\def\sautpage{\vadjust{\pagebreak}}
\newcommand\PB{\pagebreak}
\newcommand\SP{\sautpage}
\newcommand\SPB{\sautpage\break}
\newcommand\PBI{\pagebreak\noindent}


\endinput


%% predefined macros
\let\le\leqslant
\let\ge\geqslant 
\let\leq\leqslant   
\let\geq\geqslant
\let\emptyset\varnothing
\def\sfrac#1#2{{#1}/{#2}}
\def\loccit{loc.\kern3pt cit.\kern.3em}
\def\cf{cf.\kern.3em}
\def\eg{e.g.\kern.3em}
\def\ie{i.e.\kern.3em}
\def\resp{\text{resp.}\kern.3em}
\def\etc{etc.\kern.3em}
\let\ecc\etc
\let\oldsetminus\setminus
\let\setminus\smallsetminus
\newcommand{\arXiv}[1]{\href{http://arxiv.org/abs/#1}{\texttt{arXiv\string:\allowbreak#1}}}
\newcommand{\eprintHal}[1]{\href{https://hal.archives-ouvertes.fr/hal-#1}{\texttt{hal-#1}}}

\AtEndOfClass{%
\let\oldbigoplus\bigoplus
\let\oldbigcup\bigcup
\let\oldbigcap\bigcap
\let\oldbigotimes\bigotimes
\let\oldbigwedge\bigwedge
\let\oldcoprod\coprod
\def\sautpage{\vadjust{\pagebreak}}
\newcommand\PB{\pagebreak}
\newcommand\SP{\sautpage}
\newcommand\SPB{\sautpage\break}
\newcommand\PBI{\pagebreak\noindent}
}
\AtBeginDocument{%
\url@samestyle
\def\bigoplus{\mathop{\textstyle\oldbigoplus}\displaylimits}%
\def\bigcup{\mathop{\textstyle\oldbigcup}\displaylimits}%
\def\bigcap{\mathop{\textstyle\oldbigcap}\displaylimits}%
\def\bigotimes{\mathop{\textstyle\oldbigotimes}\displaylimits}%
\def\bigwedge{\mathop{\textstyle\oldbigwedge}\displaylimits}%
\def\coprod{\mathop{\textstyle\oldcoprod}\displaylimits}%
}

